Output Scaling: YingLong-Delayed Chain of Thought in a Large Pretrained Time Series Forecasting Model

We present a joint forecasting framework for time series prediction that contrasts with traditional direct or recursive methods. This framework achieves state-of-the-art performance for our designed foundation model, YingLong, and reveals a novel scaling effect: longer outputs significantly enhance model accuracy due to delayed chain-of-thought reasoning in our non-causal approach. YingLong is a non-causal, bidirectional attention encoder-only transformer trained through masked token recovery, aligning more effectively with language understanding tasks than with generation tasks. Additionally, we boost performance by tackling output variance with a multi-input ensemble. We release four foundation models ranging from 6M to 300M parameters, demonstrating superior results in zero-shot tasks on the ETT and Weather datasets. YingLong achieves more than 60% best performance. To ensure generalizability, we assessed the models using the GIFT-Eval benchmark, which comprises 23 time series datasets across 7 domains. Yinglong significantly outperformed the best time-series foundation models, end-to-end trained models by 14% and 44% in rank respectively.The pretrained 300M model is available at https://huggingface.co/qcw1314/YingLong_300m

==> sections/7_impact_statement.tex <==
\section*{Impact Statement}
This paper presents work whose goal is to advance the field of 
Time Series Forecasting. There are many potential societal consequences 
of our work, none which we feel must be specifically highlighted here.

==> tables/GIFT_Eval_domain.tex <==
\begin{table*}[htp]
\centering
\caption{Results on GIFT-Eval aggregated by domain. The best results across each row are \textbf{bolded}, while the second best results are \underline{underlined}.}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{|l|l|cccc|cccccc|cccccc|l|}
\hline
\rowcolor[HTML]{FFFFFF} 
Domain & Metric & Nv. & S. Nv. & A. Ar. & A. Th. & DeepAR & TFT & TiDE & N-BEATS & P.TST & iTrans. & T.FM & Vis.TS & $Chr_{.L}$ & $Chr_{.B}$ &$Moi_{.B}$ & $Moi_{.L}$ & \textbf{Best} \\ \hline
Econ/Fin & MAPE & 1.22 & 1.00 & 9.37e-1 & 1.01 & 1.23 & 1.14 & 1.15 & \underline{8.63e-1} & \textbf{9.46e-1} & 1.02 & 8.41e-1 & 9.93e-1 & 7.99e-1 & \underline{8.02e-1} & 1.27 & 8.80e-1 & $Chr_{.L}$ \\  
 & CRPS & 1.36 & 1.00 & 8.25e-1 & 1.36 & 1.41 & 8.48e-1 & 1.09 & \underline{9.86e-1} & \textbf{8.15e-1} & 8.55e-1 & \textbf{7.29e-1} & 1.06 & 7.74e-1 & 7.68e-1 & 1.04 & 7.36e-1 & T.FM \\  
 & Rank & 15.17 & 14.83 & 7.17 & 7.83 & 14.33 & 7.83 & 17.00 & 12.67 & 6.67 & 8.33 & 4.83 & 16.50 & 7.00 & 6.33  & 15.50 & 3.17& $Moi_{.L}$ \\ \hline
Energy & MAPE & 1.23 & 1.00 & 1.02 & 1.35 & \textbf{1.68} & 1.09 & 1.30 & 1.12 & 1.15 & 1.12 & 9.90e-1 & 1.15 & 9.12e-1 & 9.09e-1  & 9.87-1 & 8.91e-1& $Moi_{.L}$ \\  
 & CRPS & 1.72 & 1.00 & 8.63e-1 & 2.29 & 1.37 & 6.70e-1 & \textbf{8.82e-1} & \underline{9.80e-1} & \textbf{6.52e-1} & 8.26e-1 & \textbf{7.04e-1} & 8.25e-1 & 6.59e-1 & 6.61e-1  & 6.35e-1 & 6.26e-1& $Moi_{.L}$ \\  
 & Rank & 18.22 & 15.84 & 12.28 & 16.91 & 14.69 & 7.28 & 10.47 & 15.09 & 5.75 & 7.06 & 8.25 & 13.09 & 7.25 & 7.38  & 5.68 & 5.38& $Moi_{.L}$ \\ \hline
Healthcare & MAPE & 1.21 & 1.00 & 7.83e-1 & \underline{8.57e-1} & \textbf{7.90e-1} & 8.43e-1 & 7.70e-1 & \underline{7.95e-1} & 8.94e-1 & 9.02e-1 & \textbf{7.91e-1} & 8.03e-1 & 6.62e-1 & 7.25e-1  & 1.15 & 8.17e-1& $Chr_{.L}$ \\  
 & CRPS & 1.29 & 1.00 & 6.31e-1 & \underline{8.64e-1} & \textbf{7.01e-1} & 8.43e-1 & 1.07 & \underline{8.69e-1} & \textbf{5.94e-1} & 7.56e-1 & 7.99e-1 & 7.96e-1 & \underline{5.31e-1} & \underline{5.97e-1}  & 1.07 & 6.86e-1& $Chr_{.L}$ \\  
 & Rank & 17.80 & 15.00 & 7.80 & 12.00 & 14.00 & 12.40 & 10.40 & 15.80 & 8.00 & 9.40 & 7.80 & 12.80 & 4.20 & \textbf{5.00}  & 15.8 & 8.00& $Chr_{.L}$ \\ \hline
Nature & MAPE & 1.02 & 1.00 & 9.36e-1 & \textbf{1.34} & 1.35 & 1.65 & \textbf{2.05} & 9.76e-1 & \underline{1.02} & 1.02 & 1.08 & 1.04 & 7.22e-1 & \textbf{8.09e-1}  & 1.08 & 9.01e-1& $Chr_{.L}$ \\  
 & CRPS & 1.52 & 1.00 & \underline{7.10e-1} & 1.02 & 7.84e-1 & \textbf{4.02e-1} & 6.49e-1 & 5.87e-1 & 4.04e-1 & 3.92e-1 & \textbf{3.82e-1} & 4.87e-1 & 4.33e-1 & 4.35e-1  & 4.22e-1 & 3.78e-1& $Moi_{.L}$ \\  
 & Rank & 19.27 & 18.60 & 14.40 & 16.40 & 11.87 & 7.47 & 13.47 & 14.53 & 7.27 & 6.53 & 5.73 & 11.67 & 8.20 & 8.73  & 4.47 & 4.13& $Moi_{.L}$ \\ \hline
Sales & MAPE & 9.99e-1 & 1.00 & 7.72e-1 & 7.39e-1 & 7.57e-1 & 1.00 & \underline{7.60e-1} & \textbf{7.51e-1} & 6.68e-1 & 7.59e-1 & 6.83e-1 & \underline{8.11e-1} & \textbf{7.03e-1} & \textbf{6.71e-1}  & 6.68e-1 & 6.71e-1& $Moi_{.B}$ \\  
 & CRPS & 9.35e-1 & 1.00 & 4.83e-1 & 3.68e-1 & 3.64e-1 & 1.00 & \underline{4.26e-1} & \textbf{3.25e-1} & 3.64e-1 & 3.71e-1 & 3.65e-1 & 5.23e-1 & \underline{3.84e-1} & \underline{3.58e-1}  & 5.16e-1 & 4.06e-1& TFT \\  
 & Rank & 19.00 & 19.25 & 14.25 & 10.75 & 8.40 & 2.00 & 14.00 & 11.00 & 5.25 & 4.75 & \textbf{2.75} & 15.50 & 7.25 & 7.25  & 9.00 & 5.25& T.FM \\ \hline
Transport & MAPE & 1.48 & 1.00 & 1.07 & 1.08 & 8.11e-1 & 8.22e-1 & 8.78e-1 & \underline{7.60e-1} & 8.02e-1 & 8.27e-1 & 9.28e-1 & 8.70e-1 & 8.47e-1 & 8.53e-1  & 8.56e-1 & 9.28e-1& N-BEATS \\  
 & CRPS & 2.29 & 1.00 & 7.90e-1 & 1.48 & \underline{9.85e-1} & \textbf{5.00e-1} & \textbf{4.78e-1} & 5.02e-1 & 4.78e-1 & 5.00e-1 & 5.78e-1 & 6.66e-1 & 5.85e-1 & 5.86e-1  & 4.78e-1 & 5.02e-1& $Moi_{.B}$ \\  
 & Rank & 20.13 & 17.33 & 15.87 & 18.73 & 12.07 & 4.67 & 10.40 & 12.60 & 6.67 & 5.87 & 13.67 & 8.40 & 8.07 & 5.33  & 6.13 & 6.67& TFT \\ \hline
Web/CloudOps & MAPE & 1.11 & 1.00 & 8.94e-1 & 8.33e-1 & \textbf{8.57e-1} & 1.35 & 9.58e-1 & \underline{6.42e-1} & \textbf{6.02e-1} & 9.04e-1 & 2.37 & 8.38e-1 & \textbf{1.33} & 1.30  & 1.06 & 7.91e-1& P.TST \\  
 & CRPS & 1.19 & 1.00 & 9.24e-1 & 7.38e-1 & 7.81e-1 & 6.49e-1 & 6.73e-1 & 6.62e-1 & \textbf{5.18e-1} & 5.22e-1 & 9.76e-1 & 7.24e-1 & 7.91e-1 & 8.11e-1  & 7.68e-1 & 7.42e-1& P.TST \\  
 & Rank & 16.70 & 16.35 & 14.50 & 10.70 & 11.70 & 11.70 & 10.65 & 10.30 & 8.35 & 4.50 & 11.20 & 9.95 & 11.65 & 11.35  & 9.25 & 8.35& P.TST \\ \hline
\end{tabular}
}
\end{table*}

==> tables/GIFT_eval_all_update.tex <==
\vskip -0.05in
\begin{table}[ht]
\centering
\caption{Results on GIFT-Eval (Best: \textcolor{red}{Red}, Second: \textcolor{blue}{Blue})}
\label{tab:gift_eval:main}
\resizebox{0.7\textwidth}{!}{ % Resize table to fit the width of the text
\setlength{\tabcolsep}{6pt} % Adjust cell padding
\renewcommand{\arraystretch}{1.2} % Increase row height
\begin{tabular}{@{}>{\columncolor[gray]{0.9}}lccc|>{\columncolor[gray]{0.95}}cccc}
\toprule
\multicolumn{4}{c}{\cellcolor[gray]{0.8}\textbf{Foundation Model}} & 
\multicolumn{4}{c}{\cellcolor[gray]{0.8}\textbf{End-to-end and Statistical}} \\
\midrule
%\cmidrule(lr){1-4}\cmidrule(lr){5-8} \\
Model & MASE & CRPS & Rank & Model & MASE & CRPS & Rank\\
\midrule
\textsc{YINGLONG}$_{300m}$ & \textcolor{blue}{0.716} & \textcolor{red}{0.463} & \textcolor{red}{7.38} & PatchTST & 0.762 & 0.496& 10.61 \\
\textsc{YINGLONG}$_{110m}$ & 0.726 & 0.471 & \textcolor{blue}{8.04} & iTransformer & 0.802 & 0.524 & 11.90  \\
chronos-bolt$_b$  & 0.725 & 0.485 & 8.61  & TFT & 0.822 & 0.511 &12.03 \\
\textsc{YINGLONG}$_{50m}$& 0.738 & 0.479 & 8.74  & TIDE & 0.980 & 0.652&19.22 \\
TabPFN-TS &0.748 & 0.480 & 8.88 & DeepAR & 1.206 & 0.721 &19.43\\
TimesFM2$_{500m}$ &\textcolor{red}{0.680} & \textcolor{blue}{0.465} & 8.90 & Crossformer & 2.310 & 1.383 &21.47\\
chronos-bolt$_s$&0.738 & 0.487 & 9.36 & N-BEATS & 0.842 & 0.689 &21.92\\
Moirai$_{\textrm{large}}$  & 0.785 & 0.506 & 10.71& Lag-Llama & 1.101 & 0.744 &22.34\\
 Moirai$_{\textrm{base}}$   & 0.809 & 0.515 & 10.83 & DLinear & 0.952 & 0.714 &23.56\\
 \textsc{YINGLONG}$_{6m}$   & 0.790 & 0.515 & 12.55 &  &  &  & \\
Moirai$_{\textrm{small}}$  & 0.849 & 0.549 & 14.17 &  &  &  & \\
Chronos$_{\textrm{large}}$ & 0.781 & 0.547 & 14.74 &  &  &  & \\
Chronos$_{\textrm{base}}$  & 0.786 & 0.550 & 14.84 &  &  &  & \\
TimesFM                    & 0.967 & 0.575 & 15.09 &  &  &  & \\
Chronos$_{\textrm{small}}$ & 0.800 & 0.560 & 15.85 & Auto Arima & 0.964 & 0.770 &21.91\\
VisionTS                   & 0.775 & 0.638 & 21.02 & Auto Theta & 0.978 & 1.051&24.34\\
Lag-Llama                  & 1.101 & 0.744 & 22.34 & Auto ETS & 1.088 & 6.327&25.21 \\
TTMs                       & 0.969 & 0.753 & 24.04 & Seasonal Naive & 1.00 & 1.00&26.36 \\
Timer                      & 1.019 & 0.820 & 25.67 & Naive & 1.260 & 1.383 &28.24\\
\bottomrule
\end{tabular}
} % End resizebox
\vskip -0.3in
\end{table}


==> tables/in_distribution_full.tex <==
\begin{table*}[htp]
  \centering
  \caption{Full results of in-domain forecasting experiments. A lower MSE or MAE indicates a better prediction. 
  Full-shot results besides the Global Temp dataset, the TFT and N-Beats models are obtained from \citep{liuitransformer}. 
  {\boldres{Red}}: the best, \secondres{Blue}: the 2nd best.}
  \resizebox{1\columnwidth}{!}{
    %\renewcommand{\arraystretch}{1.1}
    \renewcommand{\tabcolsep}{3pt}
    \begin{tabular}{cr|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
          \toprule
            \multicolumn{2}{c}{\multirow{3}{*}{\scalebox{1.2}{\textbf{Models}}}}       & \multicolumn{6}{c}{\emoji{figures/timemoe-logo.png} \textbf{\method (Ours)}}                 & \multicolumn{20}{c}{\emoji{figures/full-shot.png} \textbf{Full-shot Time Series Models}} \\
          \cmidrule(lr){3-8} \cmidrule(lr){9-28}
          &       & \multicolumn{2}{c}{\textbf{{\basemodel}}} & \multicolumn{2}{c}{\textbf{{\largemodel}}} & \multicolumn{2}{c}{\textbf{{\ultramodel}}} & \multicolumn{2}{c}{\textbf{iTransformer}} & \multicolumn{2}{c}{\textbf{TimeMixer}} &  \multicolumn{2}{c}{\textbf{TimesNet}} & \multicolumn{2}{c}{\textbf{PatchTST}} & \multicolumn{2}{c}{\textbf{Crossformer}} & \multicolumn{2}{c}{\textbf{TiDE}} & \multicolumn{2}{c}{\textbf{DLinear}} & \multicolumn{2}{c}{\textbf{FEDformer}} & \multicolumn{2}{c}{\textbf{TFT}} & \multicolumn{2}{c}{\textbf{N-BEATS}} \\

          \cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}\cmidrule(lr){17-18}\cmidrule(lr){19-20} \cmidrule(lr){21-22} \cmidrule(lr){23-24} \cmidrule(lr){25-26} \cmidrule(lr){27-28}
          
          \multicolumn{2}{c}{\scalebox{1.2}{\textbf{Metrics}}}& \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} \\
          \midrule    \multirow{4}[1]{*}{ETTh1} & 96    & 0.345 & 0.373 & \secondres{0.335} & \secondres{0.371} & \boldres{0.323} & \boldres{0.365} & 0.386 & 0.405 & 0.375 & 0.400 & 0.384 & 0.402 & 0.414 & 0.419 & 0.423 & 0.448 & 0.479 & 0.464 & 0.386 & 0.400 & 0.376 & 0.419 & 0.478 & 0.476 & 0.383 & 0.405 \\
          & 192   & \secondres{0.372} & \secondres{0.396} & 0.374 & 0.400 & \boldres{0.359} & \boldres{0.391} & 0.441 & 0.436 & 0.436 & 0.429 & 0.421 & 0.429 & 0.460 & 0.445 & 0.471 & 0.474 & 0.525 & 0.492 & 0.437 & 0.432 & 0.420 & 0.448 & 0.510 & 0.486 & 0.453 & 0.447 \\
          & 336   & \secondres{0.389} & \boldres{0.412} & 0.390 & \boldres{0.412} & \boldres{0.388} & \secondres{0.418} & 0.487 & 0.458 & 0.484 & 0.458 & 0.491 & 0.469 & 0.501 & 0.466 & 0.570 & 0.546 & 0.565 & 0.515 & 0.481 & 0.459 & 0.459 & 0.465 & 0.548 & 0.505 & 0.517 & 0.493 \\
          & 720   & \secondres{0.410} & \secondres{0.443} & \boldres{0.402} & \boldres{0.433} & 0.425 & 0.450 & 0.503 & 0.491 & 0.498 & 0.482 & 0.521 & 0.500 & 0.500 & 0.488 & 0.653 & 0.621 & 0.594 & 0.558 & 0.519 & 0.516 & 0.506 & 0.507 & 0.549 & 0.515 & 0.594 & 0.546 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} &0.379 & \secondres{0.406} & \secondres{0.375} & \boldres{0.404} & \boldres{0.373} & \secondres{0.406} & 0.454 & 0.447 & 0.448 & 0.442 & 0.454 & 0.450 & 0.468 & 0.454 & 0.529 & 0.522 & 0.540 & 0.507 & 0.455 & 0.451 & 0.440 & 0.459 & 0.521 & 0.496 & 0.487 & 0.473 \\
    \midrule
    \multirow{4}[0]{*}{ETTh2} &96    & \secondres{0.276} & \secondres{0.340} & 0.278 & \boldres{0.335} & \boldres{0.274} & 0.338 & 0.297 & 0.349 & 0.289 & 0.341 & 0.340 & 0.374 & 0.302 & 0.348 & 0.745 & 0.584 & 0.400 & 0.440 & 0.333 & 0.387 & 0.358 & 0.397 & 0.352 & 0.387 & 0.362 & 0.384 \\
          & 192   & \secondres{0.331} & \secondres{0.371} & 0.345 & 0.373 & \boldres{0.330} & \boldres{0.370} & 0.380 & 0.400 & 0.372 & 0.392  & 0.402 & 0.414 & 0.388 & 0.400 & 0.877 & 0.656 & 0.528 & 0.509 & 0.477 & 0.476 & 0.429 & 0.439 & 0.429 & 0.432 & 0.413 & 0.430 \\
          & 336   & \secondres{0.373} & \secondres{0.402} & 0.384 & \secondres{0.402} & \boldres{0.362} & \boldres{0.396} & 0.428 & 0.432 & 0.386 & 0.414 & 0.452 & 0.541 & 0.426 & 0.433 & 1.043 & 0.731 & 0.643 & 0.571 & 0.594 & 0.541 & 0.496 & 0.487 & 0.461 & 0.460 & 0.430 & 0.448 \\
          & 720   & \secondres{0.404} & \secondres{0.431} & 0.437 & 0.437 & \boldres{0.370} & \boldres{0.417} & 0.427 & 0.445  & 0.412 & 0.434 & 0.462 & 0.657 & 0.431 & 0.446 & 1.104 & 0.763 & 0.874 & 0.679 & 0.831 & 0.657 & 0.463 & 0.474 & 0.475 & 0.473 & 0.554 & 0.530 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & \secondres{0.346} & \secondres{0.386} & 0.361 & \secondres{0.386} & \boldres{0.334} & \boldres{0.380} & 0.383 & 0.406 & 0.364 & 0.395 & 0.414 & 0.496 & 0.386 & 0.406 & 0.942 & 0.683 & 0.611 & 0.549 & 0.558 & 0.515 & 0.436 & 0.449 & 0.429 & 0.438 & 0.440 & 0.448 \\ 
    \midrule
    \multirow{4}[0]{*}{ETTm1} & 96    & 0.286 & 0.334 & \secondres{0.264} & \secondres{0.325} & \boldres{0.256} & \boldres{0.323} & 0.334 & 0.368 & 0.320 & 0.357 & 0.338 & 0.375 & 0.329 & 0.367 & 0.404 & 0.426 & 0.364 & 0.387 & 0.345 & 0.372 & 0.379 & 0.419  & 0.468 & 0.444 & 0.334 & 0.372 \\
          & 192   & 0.307 & 0.358 & \secondres{0.295} & \secondres{0.350} & \boldres{0.281} & \boldres{0.343} & 0.377 & 0.391 & 0.361 & 0.381 & 0.374 & 0.387 & 0.367 & 0.385 & 0.450 & 0.451 & 0.398 & 0.404 & 0.380 & 0.389  & 0.426 & 0.441 & 0.557 & 0.488 & 0.379 & 0.401 \\
          & 336   & 0.354 & 0.390 & \boldres{0.323} & \secondres{0.376} & \secondres{0.326} & \boldres{0.374} & 0.426 & 0.420 & 0.390 & 0.404  & 0.410 & 0.411 & 0.399 & 0.410 & 0.532 & 0.515 & 0.428 & 0.425 & 0.413 & 0.413 & 0.445 & 0.459 & 0.682 & 0.528 & 0.421 & 0.425 \\
          & 720   & \secondres{0.433} & 0.445 & \boldres{0.409} & \boldres{0.435} & 0.454 & 0.452 & 0.491 & 0.459 & 0.454 & \secondres{0.441} & 0.478 & 0.450 & 0.454 & 0.439 & 0.666 & 0.589 & 0.487 & 0.461 & 0.474 & 0.453 & 0.543 & 0.490 & 0.722 & 0.565 & 0.476 & 0.471 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & 0.345 & 0.381 & \boldres{0.322} & \boldres{0.371} & \secondres{0.329} & \secondres{0.373} & 0.407 & 0.409 & 0.381 & 0.395 & 0.400 & 0.405 & 0.387 & 0.400 & 0.513 & 0.495 & 0.419 & 0.419 & 0.403 & 0.406 & 0.448 & 0.452 & 0.607 & 0.506 & 0.403 & 0.417 \\           
    \midrule
    \multirow{4}[0]{*}{ETTm2} & 96    & \secondres{0.172} & 0.265 & \boldres{0.169} & \secondres{0.259} & 0.183 & 0.273 & 0.180 & 0.264 & 0.175 & \boldres{0.258} & 0.187 & 0.267 & 0.175 & \secondres{0.259} & 0.287 & 0.366 & 0.207 & 0.305 & 0.193 & 0.292 & 0.203 & 0.287 & 0.223 & 0.295 & 0.208 & 0.283 \\
          & 192   & \secondres{0.228} & 0.306 & \boldres{0.223} & \boldres{0.295} & \boldres{0.223} & 0.301 & 0.250 & 0.309   & 0.237 & \secondres{0.299} & 0.249 & 0.309 & 0.241 & 0.302 & 0.414 & 0.492   & 0.290 & 0.364 & 0.284 & 0.362 & 0.269 & 0.328 & 0.281 & 0.329 & 0.344 & 0.372 \\
          & 336   & \secondres{0.281} & 0.345 & 0.293 & 0.341 & \boldres{0.278} & \boldres{0.339} & 0.311 & 0.348   & 0.298 & \secondres{0.340} & 0.321 & 0.351 & 0.305 & 0.343 & 0.597 & 0.542   & 0.377 & 0.422 & 0.369 & 0.427 & 0.325 & 0.366 & 0.364 & 0.373 & 0.354 & 0.383 \\
          & 720   & 0.403 & 0.424 & 0.451 & 0.433 & 0.425 & 0.424 & 0.412 & 0.407   & \boldres{0.391} & \boldres{0.396} & 0.408 & 0.403 & \secondres{0.402} & \secondres{0.400} & 1.730 & 1.042 & 0.558 & 0.524 & 0.554 & 0.522 & 0.421 & 0.415 & 0.475 & 0.435 & 0.460 & 0.455\\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & \boldres{0.271} & 0.335 & 0.284 & 0.332 & 0.277 & 0.334 & 0.288 & 0.332 & \secondres{0.275} & \boldres{0.323} & 0.291 & 0.332 & 0.280 & \secondres{0.326} & 0.757 & 0.610 & 0.358 & 0.403 & 0.350 & 0.400 & 0.304 & 0.349 & 0.336 & 0.358 & 0.342 & 0.373 \\                      
    \midrule
    \multirow{4}[0]{*}{Weather} & 96    & \secondres{0.151} & \secondres{0.203} & \boldres{0.149} & \boldres{0.201} & 0.154 & 0.208 & 0.174 & 0.214 & 0.163 & 0.209 & 0.172 & 0.220 & 0.177 & 0.218 & 0.158 & 0.230 & 0.202 & 0.261 & 0.196 & 0.255 & 0.217 & 0.296 & 0.186 & 0.231 & 0.165 & 0.224 \\
          & 192   & \secondres{0.195} & \secondres{0.246} & \boldres{0.192} & \boldres{0.244} & 0.202 & 0.251 & 0.221 & 0.254 & 0.208 & 0.250 & 0.219 & 0.261 & 0.225 & 0.259 & 0.206 & 0.277 & 0.242 & 0.298 & 0.237 & 0.296  & 0.276 & 0.336 & 0.240 & 0.275 & 0.209 & 0.269 \\
          & 336   & \secondres{0.247} & 0.288 & \boldres{0.245} & \boldres{0.285} & 0.252 & \secondres{0.287} & 0.278 & 0.296 & 0.251 & \secondres{0.287} & 0.280 & 0.306 & 0.278 & 0.297 & 0.272 & 0.335 & 0.287 & 0.335 & 0.283 & 0.335 & 0.339 & 0.380 & 0.302 & 0.317 & 0.261 & 0.310 \\
          & 720   & \secondres{0.352} & 0.366 & \secondres{0.352} & 0.365 & 0.392 & 0.376 & 0.358 & \secondres{0.349} & 0.339 & \boldres{0.341} & 0.365 & 0.359 & 0.354 & 0.348 & 0.398 & 0.418 & 0.351 & 0.386 & 0.345 & 0.381 & 0.403 & 0.428 & 0.388 & 0.369 & \boldres{0.336} & 0.362 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & \secondres{0.236} & 0.275 & \boldres{0.234} & \secondres{0.273} & 0.250 & 0.280 & 0.257 & 0.278 & 0.240 & \boldres{0.271} & 0.259 & 0.286 & 0.258 & 0.280 & 0.258 & 0.315 & 0.270 & 0.320 & 0.265 & 0.316 & 0.308 & 0.360 & 0.279 & 0.298 & 0.243 & 0.291  \\   
    \midrule
     \multirow{4}[0]{*}{Global Temp} & 96    & \secondres{0.192} & \secondres{0.328} & \secondres{0.192} & 0.329 & \boldres{0.189} & \boldres{0.322}  & 0.223 & 0.351 & 0.215 & 0.346 & 0.250 & 0.381 & 0.219 & 0.349 & 0.272 & 0.406 & 0.223 & 0.352 & 0.221 & 0.354 & 0.261 & 0.392 & 0.260 & 0.390 & 0.210 & 0.344 \\
          & 192   & 0.238 & \boldres{0.375} & \secondres{0.236} &\boldres{ 0.375} & \boldres{0.234} & \secondres{0.376} & 0.282 & 0.404 & 0.266 & 0.393 & 0.298 & 0.418 & 0.269 & 0.395 & 0.305 & 0.435 & 0.278 & 0.401 & 0.257 & 0.388 & 0.299 & 0.423 & 0.301 & 0.423 & 0.253 & 0.385 \\
          & 336   & 0.259 & \boldres{0.397} & \secondres{0.256} & \boldres{0.397} & \boldres{0.253} & \secondres{0.399} & 0.313 & 0.431 & 0.313 & 0.430 & 0.315 & 0.434 & 0.319 & 0.435 & 0.352 & 0.468 & 0.330 & 0.440 & 0.294 & 0.418 & 0.341 & 0.454 & 0.359 & 0.464 & 0.282 & 0.411 \\
          & 720   & 0.345 & 0.465  & \secondres{0.322} & \secondres{0.451} & \boldres{0.292} & \boldres{0.426} & 0.393 & 0.488 & 0.468 & 0.536 & 0.407 & 0.497 & 0.452 & 0.526 & 0.508 & 0.562 & 0.485 & 0.544 & 0.380 & 0.479 & 0.359 & 0.469 & 0.371 & 0.477 & 0.342 & 0.457 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & 0.258 & 0.391 & \secondres{0.251} & \secondres{0.388} & \boldres{0.242} & \boldres{0.380} & 0.303 & 0.419 & 0.316 & 0.426 & 0.318 & 0.433 & 0.315 & 0.426 & 0.359 & 0.468 & 0.329 & 0.434 & 0.288 & 0.410 & 0.315 & 0.435 & 0.323 & 0.439 & 0.272 & 0.399 \\  
    \midrule
    \rowc\rowcolor{blue!15}
    \multicolumn{2}{c|}{\scalebox{1.1}
    {\textbf{Average}}} & 0.306 & 0.362 & \secondres{0.304} & \secondres{0.359} & \boldres{0.301} & \boldres{0.358} & 0.349 & 0.382 & 0.337 & 0.375 & 0.356 & 0.400 & 0.349 & 0.382 & 0.560 & 0.516 & 0.421 & 0.439 & 0.387 & 0.416 & 0.375  & 0.417 & 0.416 & 0.422 & 0.364 & 0.400\\
    \midrule
    \rowc
    \multicolumn{2}{c}{\textbf{{$1^{\text{st}}$ Count}}} & \multicolumn{2}{c}{4} & \multicolumn{2}{c}{\secondres{21}} & \multicolumn{2}{c}{\boldres{33}} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{6} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} &  \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{0} & \multicolumn{2}{c}{1} \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:lsf_full}%
\end{table*}%



==> tables/related_work.tex <==
\vspace{-3mm}
\begin{table*}[ht]
  \caption{Comparison between large time series models.}
  \vspace{-2pt}
  \label{tab:ltsm_comp}
  \centering
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{1pt}
  % \renewcommand\arraystretch{1.3}
  \resizebox{1.6\columnwidth}{!}{
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
    \toprule
    Method & YinLong& Time-MoE & Moirai & TimesFM & Moment & Chronos & Timer & Lag-Llama & TimeGPT   \\ 
    \toprule
     \multirow{2}{*}{Architecture} &Encoder-& Decoder- & Encoder-  & Decoder- & Encoder- & Encoder-  & Decoder- & Decoder- & Encoder-\\
     &Only & Only & Only & Only & Only & Decoder & Only & Only & Decoder \\
    \midrule
    (Max) Model Size &300M & 2.4B & 311M & 200M & 385M & 710M & 67M & 200M & Unknown \\
    \midrule
    Input Token &Patch & Point & Patch & Patch & Patch & Point & Patch & Point & Patch \\
    % \midrule
    % Dataset Scale& & 309B & 27B/231B\textsuperscript{*} & 100B & 1.13B & 84B & 28B & 0.36B & 100B \\
    \midrule
    Max Context Length& 8192 & 4096 & 5000 & 512 & 512  & 512 & 1440 & 1024 & Unknown \\
    % \midrule
    % Open-source Data&\checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark &  &   \\
    \midrule
    Output scaling&\checkmark &  &  &  &  &  &  &  &   \\
    \midrule
    Multi-Input ensemble &\checkmark &  &  &  &  &  &  &  &   \\
    % \midrule
    % Source & Ours & \citeauthor{shi2024time} & \footnotesize\citeauthor{woo2024unified} & \footnotesize\citeauthor{dasdecoder} & \fontsize{8.5pt}{10pt}\selectfont\citeauthor{goswamimoment} & \footnotesize\citeauthor{ansari2024chronos} & \footnotesize\citeauthor{liutimer} & \footnotesize\citeauthor{rasul2023lagllama} & \footnotesize\citeauthor{garza2023timegpt} \\
    \bottomrule
    % \multicolumn{9}{l}{\textsuperscript{*} \small{Depend on the way of calculation according to the original paper.}}
  \end{tabular}
  }
  \vspace{-2pt}
\end{table*}

==> tables/zero_full.tex <==
\vspace{-3mm}
\begin{table*}[htbp]
  \centering
  \caption{Full results of zero-shot forecasting experiments. A lower MSE or MAE indicates a better prediction. TimesFM, due to its use of Weather datasets in pretraining, is not evaluated on this dataset and is denoted by a dash ($-$). {\boldres{Red}}: the best, \secondres{Blue}: the 2nd best.} %The below table represents these results by a dash ($-$).}
  \resizebox{2\columnwidth}{!}{
    \renewcommand{\tabcolsep}{3pt}
    \begin{tabular}{cr|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
          \toprule
          \multicolumn{2}{c}{\multirow{3}{*}{\textbf{\scalebox{1.2}{Models}}}} &\multicolumn{6}{c}{\emoji{figures/timemoe-logo.png} \textbf{\method (Ours)}}& \multicolumn{16}{c}{\emoji{figures/zero-shot.png} \textbf{Zero-shot Time Series Models}} \\
          \cmidrule(lr){3-8} \cmidrule(lr){9-24}
          &       & \multicolumn{2}{c}{\textbf{{\basemodel}}} & \multicolumn{2}{c}{\textbf{{\largemodel}}} & \multicolumn{2}{c}{\textbf{{\ultramodel}}} & \multicolumn{2}{c}{\textbf{Moirai$_{small}$}} & \multicolumn{2}{c}{\textbf{Moirai$_{base}$}} & \multicolumn{2}{c}{\textbf{Moirai$_{large}$}} & \multicolumn{2}{c}{\textbf{TimesFM}} & \multicolumn{2}{c}{\textbf{Moment}} & \multicolumn{2}{c}{\textbf{Chronos$_{small}$}} & \multicolumn{2}{c}{\textbf{Chronos$_{base}$}} & \multicolumn{2}{c}{\textbf{Chronos$_{large}$}} \\
          % \midrule
          \cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}\cmidrule(lr){17-18}\cmidrule(lr){19-20}\cmidrule(lr){21-22}\cmidrule(lr){23-24}
          
          \multicolumn{2}{c}{\scalebox{1.2}{\textbf{Metrics}}}& \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE}  \\
          \midrule    \multirow{4}[1]{*}{ETTh1} & 96    & 0.357 & \secondres{0.381} & \secondres{0.350} & 0.382 & \boldres{0.349} & \boldres{0.379} & 0.401 & 0.402 & 0.376 & 0.392 & 0.381 & 0.388 & 0.414 & 0.404 & 0.688 & 0.557 & 0.466 & 0.409 & 0.440 & 0.393 & 0.441 & 0.390 \\
          & 192   & \boldres{0.384} & \boldres{0.404} & \secondres{0.388} & \secondres{0.412} & 0.395 & 0.413 & 0.435 & 0.421 & 0.412 & 0.413 & 0.434 & 0.415 & 0.465 & 0.434 & 0.688 & 0.560 & 0.530 & 0.450 & 0.492 & 0.426 & 0.502 & 0.424 \\
          & 336   & \boldres{0.411} & 0.434 & \boldres{0.411} & \secondres{0.430} & 0.447 & 0.453 & 0.438 & 0.434 & \secondres{0.433} & \boldres{0.428} & 0.495 & 0.445 & 0.503 & 0.456 & 0.675 & 0.563 & 0.570 & 0.486 & 0.550 & 0.462 & 0.576 & 0.467 \\
          & 720   & 0.449 & 0.477 & \boldres{0.427} & 0.455 & 0.457 & 0.462 & \secondres{0.439} & \secondres{0.454} & 0.447 & \boldres{0.444} & 0.611 & 0.510 & 0.511 & 0.481 & 0.683 & 0.585 & 0.615 & 0.543 & 0.882 & 0.591 & 0.835 & 0.583 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & \secondres{0.400} & \secondres{0.424} & \boldres{0.394} & \boldres{0.419} & 0.412 & 0.426 & 0.428 & 0.427 & 0.417 & \boldres{0.419} & 0.480 & 0.439 & 0.473 & 0.443 & 0.683 & 0.566 & 0.545 & 0.472 & 0.591 & 0.468 & 0.588 & 0.466 \\
    \midrule
    \multirow{4}[0]{*}{ETTh2} & 96    & 0.305 & 0.359 & 0.302 & 0.354 & \boldres{0.292} & 0.352 & 0.297 & \secondres{0.336} & \secondres{0.294} & \boldres{0.330} & 0.296 & \boldres{0.330} & 0.315 & 0.349 & 0.342 & 0.396 & 0.307 & 0.356 & 0.308 & 0.343 & 0.320 & 0.345 \\
          & 192   & \secondres{0.351} & 0.386 & 0.364 & 0.385 & \boldres{0.347} & 0.379 & 0.368 & 0.381 & 0.365 & \secondres{0.375} & 0.361 & \boldres{0.371} & 0.388 & 0.395 & 0.354 & 0.402 & 0.376 & 0.401 & 0.384 & 0.392 & 0.406 & 0.399 \\
          & 336   & 0.391 & 0.418 & 0.417 & 0.425 & 0.406 & 0.419 & \secondres{0.370} & 0.393 & 0.376 & \boldres{0.390} & 0.390 & \boldres{0.390} & 0.422 & 0.427 & \boldres{0.356} & \secondres{0.407} & 0.408 & 0.431 & 0.429 & 0.430 & 0.492 & 0.453 \\
          & 720   & 0.419 & 0.454 & 0.537 & 0.496 & 0.439 & 0.447 & \secondres{0.411} & \secondres{0.426} & 0.416 & 0.433 & 0.423 & \boldres{0.418} & 0.443 & 0.454 & \boldres{0.395} & 0.434 & 0.604 & 0.533 & 0.501 & 0.477 & 0.603 & 0.511 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & 0.366 & 0.404 & 0.405 & 0.415 & 0.371 & 0.399 & \boldres{0.361} & 0.384 & \secondres{0.362} & \secondres{0.382} & 0.367 & \boldres{0.377} & 0.392 & 0.406 & \boldres{0.361} & 0.409 & 0.424 & 0.430 & 0.405 & 0.410 & 0.455 & 0.427 \\
    \midrule
    \multirow{4}[0]{*}{ETTm1} & 96    & 0.338 & 0.368 & \secondres{0.309} & 0.357 & \boldres{0.281} & \boldres{0.341} & 0.418 & 0.392 & 0.363 & \secondres{0.356} & 0.380 & 0.361 & 0.361 & 0.370 & 0.654 & 0.527 & 0.511 & 0.423 & 0.454 & 0.408 & 0.457 & 0.403 \\
          & 192   & 0.353 & 0.388 & \secondres{0.346} & 0.381 & \boldres{0.305} & \boldres{0.358}  & 0.431 & 0.405 & 0.388 & \secondres{0.375} & 0.412 & 0.383 & 0.414 & 0.405 & 0.662 & 0.532 & 0.618 & 0.485 & 0.567 & 0.477 & 0.530 & 0.450 \\
          & 336   & 0.381 & 0.413 & \secondres{0.373} & 0.408 & \boldres{0.369} & \secondres{0.395}  & 0.433 & 0.412 & 0.416 & \boldres{0.392} & 0.436 & 0.400 & 0.445 & 0.429 & 0.672 & 0.537 & 0.683 & 0.524 & 0.662 & 0.525 & 0.577 & 0.481 \\
          & 720   & 0.504 & 0.493 & 0.475 & 0.477 & 0.469 & 0.472  & \secondres{0.462} & 0.432 & \boldres{0.460} & \boldres{0.418} & \secondres{0.462} & \secondres{0.420} & 0.512 & 0.471 & 0.692 & 0.551 & 0.748 & 0.566 & 0.900 & 0.591 & 0.660 & 0.526 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & 0.394 & 0.415  & \secondres{0.376} & 0.405 & \boldres{0.356} & \secondres{0.391} & 0.436 & 0.410 & 0.406 & \boldres{0.385} & 0.422 & 0.391 & 0.433 & 0.418 & 0.670 & 0.536 & 0.640 & 0.499 & 0.645 & 0.500 & 0.555 & 0.465 \\
    \midrule
    \multirow{4}[0]{*}{ETTm2} & 96    & 0.201 & 0.291 & \boldres{0.197} & 0.286 & \secondres{0.198} & 0.288 & 0.214 & 0.288 & 0.205 & \secondres{0.273} & 0.211 & 0.274 & 0.202 & \boldres{0.270} & 0.260 & 0.335 & 0.209 & 0.291 & 0.199 & 0.274 & \boldres{0.197} & 0.271 \\
          & 192   & 0.258 & 0.334 & \secondres{0.250} & 0.322 & \boldres{0.235} & \boldres{0.312} & 0.284 & 0.332 & 0.275 & 0.316 & 0.281 & 0.318 & 0.289 & 0.321 & 0.289 & 0.350 & 0.280 & 0.341 & 0.261 & 0.322 & 0.254 & \secondres{0.314} \\
          & 336   & 0.324 & 0.373 & 0.337 & 0.375 & \boldres{0.293} & \boldres{0.348} & 0.331 & 0.362 & 0.329 & \secondres{0.350} & 0.341 & 0.355 & 0.360 & 0.366 & 0.324 & 0.369 & 0.354 & 0.390 & 0.326 & 0.366 & \secondres{0.313} & 0.353 \\
          & 720   & 0.488 & 0.464 & 0.480 & 0.461 & 0.427 & 0.428 & \secondres{0.402} & \boldres{0.408} & 0.437 & \secondres{0.411} & 0.485 & 0.428 & 0.462 & 0.430 & \boldres{0.394} & 0.409 & 0.553 & 0.499 & 0.455 & 0.439 & 0.416 & 0.415 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & 0.317 & 0.365  & 0.316 & 0.361 & \boldres{0.288} & 0.344 & 0.307 & 0.347 & 0.311 & \boldres{0.337} & 0.329 & 0.343 & 0.328 & 0.346 & 0.316 & 0.365 & 0.349 & 0.380 & 0.310 & 0.350 & \secondres{0.295} & \secondres{0.338} \\
    \midrule
    \multirow{4}[0]{*}{Weather} & 96    & 0.160 & 0.214 & \secondres{0.159} & \secondres{0.213} & \boldres{0.157} & \boldres{0.211} & 0.198 & 0.222 & 0.220 & 0.217 & 0.199 & \boldres{0.211} & - & - & 0.243 & 0.255 & 0.211 & 0.243 & 0.203 & 0.238 & 0.194 & 0.235 \\
          & 192   & \secondres{0.210} & 0.260 & 0.215 & 0.266 & \boldres{0.208} & \secondres{0.256} & 0.247 & 0.265 & 0.271 & 0.259 & 0.246 & \boldres{0.251} & - & - & 0.278 & 0.329 & 0.263 & 0.294 & 0.256 & 0.290 & 0.249 & 0.285 \\
          & 336   & \secondres{0.274} & 0.309 & 0.291 & 0.322 & \boldres{0.255} & \boldres{0.290} & 0.283 & 0.303 & 0.286 & 0.297 & \secondres{0.274} & \secondres{0.291} & - & - & 0.306 & 0.346 & 0.321 & 0.339 & 0.314 & 0.336 & 0.302 & 0.327 \\
          & 720   & 0.418 & 0.405 & 0.415 & 0.400 & 0.405 & 0.397 & 0.373 & 0.354 & 0.373 & \secondres{0.354} & \boldres{0.337} & \boldres{0.340} & - & - & \secondres{0.350} & 0.374 & 0.404 & 0.397 & 0.397 & 0.396 & 0.372 & 0.378 \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} &  0.265 & 0.297 & 0.270 & 0.300 & \boldres{0.256} & 0.288 & 0.275 & 0.286 & 0.287 & \secondres{0.281} & \secondres{0.264} & \boldres{0.273} & - & - & 0.294 & 0.326 & 0.300 & 0.318 & 0.292 & 0.315 & 0.279 & 0.306 \\
    \midrule
    \multirow{4}[0]{*}{Global Temp} & 96    & \secondres{0.211} & \secondres{0.343} & \boldres{0.210} & \boldres{0.342} & 0.214 & 0.345 & 0.227 & 0.354 & 0.224 & 0.351 & 0.224 & 0.351 & 0.255 & 0.375 & 0.363 & 0.472 & 0.234 & 0.361 & 0.230 & 0.355 & 0.228 & 0.354  \\
        & 192   & 0.257 & 0.386 & \secondres{0.254} & \secondres{0.385} & \boldres{0.246} & \boldres{0.379} & 0.269 & 0.396 & 0.266 & 0.394 & 0.267 & 0.395 & 0.313 & 0.423 & 0.387 & 0.489 & 0.276 & 0.400 & 0.273 & 0.395 & 0.276 & 0.398  \\
          & 336   & 0.281 & 0.405 & \secondres{0.267} & \boldres{0.395} & \boldres{0.266} & \secondres{0.398} & 0.292 & 0.419 & 0.296 & 0.420 & 0.291 & 0.417 & 0.362 & 0.460 & 0.430 & 0.517 & 0.314 & 0.431 & 0.324 & 0.434 & 0.327 & 0.437 \\
          & 720   & 0.354 & 0.465 & \secondres{0.289} & \boldres{0.420} & \boldres{0.288} & \secondres{0.421} & 0.351 & 0.437 & 0.403 & 0.498 & 0.387 & 0.488 & 0.486 & 0.545 & 0.582 & 0.617 & 0.418 & 0.504 & 0.505 & 0.542 & 0.472 & 0.535  \\
          \rowcolor{tabhighlight}
          & {\textbf{AVG}} & 0.275 & \secondres{0.400} & \secondres{0.255} & \boldres{0.385} & \boldres{0.253} & \boldres{0.385} & 0.285 & 0.409 & 0.297 & 0.416 & 0.292 & 0.413 & 0.354 & 0.451 & 0.440 & 0.524 & 0.311 & 0.424 & 0.333 & 0.431 & 0.326 & 0.431 \\
    \midrule
    \rowc\rowcolor{blue!15}
    \multicolumn{2}{c|}{\scalebox{1.1}
    {\textbf{Average}}} & \secondres{0.336} & 0.384 & \secondres{0.336} & 0.380 & \boldres{0.322} & \secondres{0.372} & 0.349 & 0.377 & 0.347 & \boldres{0.370} & 0.359 & 0.373 & 0.396 & 0.413 & 0.461 & 0.454 & 0.428 & 0.420 & 0.429 & 0.412 & 0.416 & 0.405 \\
    \midrule
    \rowc
    \multicolumn{2}{c|}{\scalebox{1.1}{\textbf{{$1^{\text{st}}$ Count}}}} & \multicolumn{2}{c|}{3} & \multicolumn{2}{c|}{10} & \multicolumn{2}{c|}{\boldres{28}} & \multicolumn{2}{c|}{2} & \multicolumn{2}{c|}{\secondres{11}} & \multicolumn{2}{c|}{10} & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{0} & \multicolumn{2}{c|}{0} & \multicolumn{2}{c}{1} \\
    \end{tabular}%
  }
  \label{tab:zero_shot_full}%
  \vspace{-2mm}
\end{table*}%
